An Exploration of Exploration: Measuring the ability of lexicase selection to find obscure pathways to optimality

Parent selection algorithms (selection schemes) steer populations through a problem's search space, often trading off between exploitation and exploration. Understanding how selection schemes affect exploitation and exploration within a search space is crucial to tackling increasingly challenging problems. Here, we introduce an "exploration diagnostic" that diagnoses a selection scheme's capacity for search space exploration. We use our exploration diagnostic to investigate the exploratory capacity of lexicase selection and several of its variants: epsilon lexicase, down-sampled lexicase, cohort lexicase, and novelty-lexicase. We verify that lexicase selection out-explores tournament selection, and we show that lexicase selection's exploratory capacity can be sensitive to the ratio between population size and the number of test cases used for evaluating candidate solutions. Additionally, we find that relaxing lexicase's elitism with epsilon lexicase can further improve exploration. Both down-sampling and cohort lexicase -- two techniques for applying random subsampling to test cases -- degrade lexicase's exploratory capacity; however, we find that cohort partitioning better preserves lexicase's exploratory capacity than down-sampling. Finally, we find evidence that novelty-lexicase's addition of novelty test cases can degrade lexicase's capacity for exploration. Overall, our findings provide hypotheses for further exploration and actionable insights and recommendations for using lexicase selection. Additionally, this work demonstrates the value of selection scheme diagnostics as a complement to more conventional benchmarking approaches to selection scheme analysis.

==> tex/scratch/2021-04-12-intro.tex <==

% - Fitness landscapes
%   - Parent selection algorithms
%   - Parent selection algorithms in the context of fitness landscapes
%   - Analyzing selection algorithms => how do they traverse the fitness landscape?
% @AML: If possible (not at all necessary for the draft), we should come back and work in 1-2 sentences about what we present/achieve in the first paragraph or two.

% JGH: If anyone has a cool paper of EAs solving hard problems feel free to cite!
Interest in evolutionary algorithms has grown over time, due to the fact that these algorithms demonstrate the ability to traverse complex fitness landscapes and produce high-quality solutions for real-world optimization problems [CITE].
As evolutionary algorithms continued to show promise with solving complex real-world optimization problems, the complexity of processes that occur during an evolutionary run also increased to solve even more difficult problems.
This is clearly illustrated when comparing an early evolutionary algorithm, such as the ES$(\mu, \lambda)$ Evolutionary Strategy, to a more modern algorithm, such as the MAP-Elites algorithm \cite{eiben1998evolutionary, mouret2015illuminating}.
While the procedural complexity within evolutionary algorithms continues to increase, many share a common step throughout their evolutionary search for high-quality solutions -- the selection scheme.

% -- Introduce fitness landscape metaphor (general) --
Fitness landscapes are useful metaphors for understanding how populations evolve [citations - malan2013survey] and how to make them evolve faster [cite - Nahum 2017].
A fitness landscape [describes] the [complex/many-dimensional] network of all possible genotypes where each genotype has an associated fitness value, and connections between genotypes represent possible mutations [that transform one genotype into the other]. 
% Evolving populations move through th
Typically, fitness landscapes are depicted as three dimensional surfaces where peaks in the landscape represent local optima, and individuals in an evolving population are represented as points on the surface, each located at its associated genotype [Figure?].
Evolving populations are clouds of points that move across the landscape as individuals reproduce, mutate, and die. 
In biological populations, [process happens as higher fitness individuals tend to be more reproductively successful/disproportionately survive relative to lower fitness individuals, moving populations up fitness peaks].

% -- Evolutionary algorithms steer populations through fitness landscapes. --
In evolutionary computing, a fitness landscape describes the search space for a given computational problem. 
In contrast to [biological evolution], evolutionary algorithms actively direct populations through a problem's search space via repeated evaluation, selection, and variation (\textit{i.e.}, replicating promising individuals with random mutations) until a sufficiently good solution is found. 
Together, each of these algorithmic components---how we represent and interpret individuals, how we select which individuals to produce offspring, and how we vary offspring---determine how an evolutionary algorithm navigates a given fitness landscape, which, in turn, determines the success of evolutionary search. 
% Many techniques exist. How do they direct populations, and how to choose which ones to use?
In this work, we focus on understanding how parent selection algorithms explore fitness landscapes.
Specifically, we introduce a selection scheme diagnostic that can be used to isolate how well a given parent selection algorithm explores fitness landscapes; we then apply our exploration diagnostic to the lexicase parent selection algorithm, [showing that...].



% - Exploration vs. exploitation
%  - Pure exploitation (greedy algorithms)
%  - Pure exploration (enumerate all possibilities)
%   - Efficient pure exploration => novelty search
% - Striking a balance between exploitation and exploration
%  - Diversity maintenance, quality diversity algorithms
Parent selection algorithms choose promising individuals in a population to contribute genetic material to the next generation based on their quality relative to one or more criteria. 
In this way, parent selection algorithms steer populations through the search space, often trading off between exploitation and exploration. 
If individuals in a population represent single points in a given search space, exploitation is the process of [evaluating] the local neighborhood of previously [discovered/evaluated] points [cite - Črepinšek]. 
Purely exploitative selection schemes (e.g., elite selection) direct populations toward the closest optimum, regardless of the optimum being global or local, and the population will not be able to escape it to explore other regions of the landscape no matter how promising those other regions might be.
Exploration is the process of [evaluating] entirely new regions of the search space [cite - Črepinšek].
Purely exploratory selection schemes (e.g., novelty search) spread populations throughout the search space, continuously [discovering] novel regions of the search space but not necessarily [climbing/identifying/steering toward] local optima. 
% is crucial to finding high quality solutions, as it is important to exploit promising regions of the fitness landscape, while also exploring the fitness landscape to find other promising regions.
The most effective selection schemes balance exploration with exploitation, exploring the fitness landscape to identify promising regions while simultaneously exploiting those promising regions to find local optima.
[Traditional selection schemes such as tournament selection and elitist selection are very exploitative.]
Different selection techniques have been created [to balance exploration and exploitation], some of which include fitness sharing, novelty search, and age-layered population structure \citep{goldberg1987genetic,lehman2011novelty,hornby2006alps}.

% Understanding how evolutionary algorithms perform exploration and exploitation within a fitness landscape is important information to have.
% As a practitioner, this information can make it possible to know what kind of evolutionary algorithm to use to meet solution requirements.
% The design of an evolutionary algorithm can dictate the trade-off between exploitation and exploration, as the selection scheme and mutation operators (point mutations, crossover, \textit{etc}.) play a role in determining the strength of each one \cite{eiben1998evolutionary}.
% Looking at an algorithm that is extremely exploitative, the algorithm will push the population to closest optimum, regardless of the optimum being global or local, and the population will not be able to escape it to explore promising regions of the landscape.
% Now looking at the other extreme, an algorithm that is extremely exploratory will spread the population across the potentially promising regions of the fitness landscape but never reach an actually optimum.
% Thus, it is clear that striking a balance between exploration and exploitation is crucial to finding high quality solutions, as it is important to exploit promising regions of the fitness landscape, while also exploring the fitness landscape to find other promising regions.
% Different techniques were also created to balance exploration and exploitation, some of which include fitness sharing, novelty search, and age-layered population structure \cite{goldberg1987genetic, lehman2011novelty, hornby2006alps}.

% -- Lexicase selection --
% - is good and useful
Lexicase-based parent selection algorithms have been proven highly successful for finding effective solutions to test-based problems in genetic programming [citations].
% - define
Lexicase-based algorithms evaluate variants on a set of tests and choose parents based on their relative performance on random permutations of the full test set; this allows variants specializing on different sequences (or prioritizations) of tests to coexist until a complete solution evolves. 
%, especially for test-based problems where there are many distinct test cases that must all be passed.
% [Commonly used in GP, but also in evolutionary robotics and learning classifier systems].
[Balances exploration with exploitation...].
% [Describe lexicase algorithm].
[Many variants].
[How do variants impact exploration].

% \textit{Lexicase-based algorithms} evaluate variants on a set of tests 
% and choose parents based on their relative performance on random permutations of the full test set; this allows variants specializing on different sequences (or prioritizations) of tests to coexist until a complete solution evolves. 

% -- benchmarking --
% - Analyzing selection algorithms with benchmarking
%   - Benchmarking
%   - Often overall problem solving success of an entire system, do not isolate selection scheme
%     - Mutation rate, representation, problem, etc
%   - Very useful in how a whole system performs in practice %   - But if our interest is to characterize selection schemes, can confound results
%   - Some benchmarking uses very stripped down/limited problems, but still don't isolate individual characteristics of a selection scheme.
[Lots of efforts to benchmark lexicase].
[E.g., ... findings ...].
[Benchmarking however often focuses on problem solving success].
[Diversity maintenance has been evaluated, ...].
[Further, benchmarking in context of entire evolutionary computing system (e.g., PushGP or XX), and exploration affected by mutation operators etc]
[Here, we propose a selection scheme \textit{diagnostic} to isolate exploration].
% One problem that occurs with using existing benchmark problems is that they too can intertwine multiple problem characteristics.
% Carefully constructing and describing novel diagnostic problems can help practitioners better understand the strengths and weaknesses of an entire evolutionary algorithm, and also how the variation of specific evolutionary algorithm components (mutation rate, mutation operator, selection scheme, \textit{etc.}) impact its problem solving success.

% In practice, it is common to evaluate an problem solving potential evolutionary algorithms to get a better understanding of its strengths and weaknesses.
% Often researchers evaluate an evolutionary algorithm on real-world optimization problems that inherently posses multiple interwoven challenging characteristics, such as conflicting objectives, deception, multi-modal, \textit{etc.}, that make it difficult to extract information about the kinds of problems it may be best suited for.
% It is possible to visualize certain optimization problems, for example if a solution consists of a two-dimensional coordinate, but it not all problems can use such a simple underlying structure.
% There is ongoing research in the field of fitness landscape analysis that focuses on the development of metrics that are able to capture characteristics that make solving an optimization problem difficult, but is limiting when the search space is extremely large \cite{malan2013survey}.
% It is also common to use both fitness landscape analysis and benchmark functions to tease apart the strengths and weaknesses of evolutionary algorithms, so that practitioners can make better decisions on which one to use \cite{sun2014selection}.
% One problem that occurs with using existing benchmark problems is that they too can intertwine multiple problem characteristics.
% Carefully constructing and describing novel diagnostic problems can help practitioners better understand the strengths and weaknesses of an entire evolutionary algorithm, and also how the variation of specific evolutionary algorithm components (mutation rate, mutation operator, selection scheme, \textit{etc.}) impact its problem solving success.

% -- What we did & our results --
% diagnostic analogies
%  - car mechanic diagnostics
%  - medical diagnostics
%  - ..?
% [What we did and our results].


% - Selection scheme diagnostics
%   - Can we diagnose different characteristics of selection schemes?
%   - Selection scheme diagnostics
%   - meant to complement benchmarking (different goal: isolate/understand characteristics of selection schemes)
%   - Introduce an *exploration* diagnostic designed to diagnose capacity for fitness landscape exploration
% JGH: I think this might have combined this in the previous paragraph

% - Use exploration diagnostic to investigate lexicase selection
%  - Verify intuition and previous benchmarking results showing that it better explores relative to tournament/mu lambda (very exploitative algorithms) 
%  - ?? number of test cases/problem decomposition?
%  - Investigate how different lexicase variants alter exploration
%    - Down-sampled
%    - Epsilon
%  - Investigate how addition of exploration-focused test cases can alter exploration
%    - Genotypic similarity (fitness sharing inspired)
%    - Age/generation (Age-layered population structure inspired)

In this work, we introduce a novel diagnostic that tests an evolutionary algorithms ability to explore multiple avenues within a fitness landscape, with the goal of finding the best avenue to pursue.
The total number of possible avenues is user dependent, so practitioners are also able to find where an algorithms exploratory abilities begin to fall off.
In particular, the algorithm of focus in this work is lexicase selection, along with other subsampling variations of it \cite{helmuth2014solving, hernandez2019random}.
We start by testing lexicase on this exploratory diagnostic with an increasing number of possible avenues to pursue to gain an understanding of its exploratory limitations.
We also evaluate how the different subsampling variations of lexicase impact an evolutionary algorithms ability to explore the exploratory diagnostic fitness landscape.
With all this information, we hope to highlight how the different variations of lexicase in this work impact an evolutionary algorithms problem solving ability when exploration is key to its success.  



==> tex/scratch/alg-cohort-lexicase.tex <==
\RestyleAlgo{boxruled}
\begin{algorithm}[h!]
    \begin{enumerate}
        \setlength\itemsep{1mm}
        \item Mark \textbf{population\_cohort} as the partitions of the population.
        \item Mark \textbf{test\_cohort} as the partitions of the \textbf{test\_cases}.
        \item For a single \textbf{population\_set} in \textbf{population\_cohort} and \textbf{test\_set} in \textbf{test\_cohort}:
        
        \begin{enumerate}
            \setlength\itemsep{1mm}
            \item Mark the entire \textbf{population\_set} as current \textbf{candidates} under consideration.
            \item Shuffle \textbf{test\_set} in a random order.
            \item For each \textbf{case} in \textbf{test\_set}: \\
            
            \begin{enumerate}
                \setlength\itemsep{1mm}
                \item Evaluate each candidate in \textbf{candidates} on \textbf{case}.
                \item Identify the \textbf{best\_score} of all candidates.
                \item Remove each entry from \textbf{candidates} with a score less than \textbf{best\_score}.
            \end{enumerate}
            
            \item Select a random entry from \textbf{candidates}.
        \end{enumerate}

    \end{enumerate}
 \caption{Cohort Lexicase Selection}
 \label{alg:cohort-lexicase}
\end{algorithm}

==> tex/scratch/alg-down-sampled-lexicase.tex <==
\RestyleAlgo{boxruled}
\begin{algorithm}[h!]
    \begin{enumerate}
        \setlength\itemsep{1mm}

        \item Set \textbf{sub\_test\_cases} to a \textbf{percentage} of cases sampled from \textbf{test\_cases}.
        
        \item Mark the entire population as current \textbf{candidates} under consideration.
        
        \item Shuffle \textbf{sub\_test\_cases} into a random order.

        \item For each \textbf{case} in \textbf{sub\_test\_cases}:
        
        \begin{enumerate}
            \setlength\itemsep{1mm}
            \item Evaluate each candidate in \textbf{candidates} on \textbf{case}.
            
            \item Identify the \textbf{best\_score} of all candidates.
            
            \item Remove each entry from \textbf{candidates} with a score less than \textbf{best\_score}.
        \end{enumerate}
        
        \item Select a random entry from \textbf{candidates}.
    \end{enumerate}
 \caption{Down-Sampled Lexicase Selection}
 \label{alg:down-sampled-lexicase}
\end{algorithm}

==> tex/scratch/alg-epsilon-lexicase.tex <==
\RestyleAlgo{boxruled}
\begin{algorithm}[h!]
    \begin{enumerate}
        \setlength\itemsep{1mm}
        
        \item Set \textbf{$\epsilon$} threshold. 
        
        \item Mark the entire population as current \textbf{candidates} under consideration.
        
        \item Shuffle \textbf{test\_cases} into a random order.

        \item For each \textbf{case} in \textbf{test\_cases}:
        \begin{enumerate}
            \setlength\itemsep{1mm}
            \item Evaluate each candidate in \textbf{candidates} on \textbf{case}.
            
            \item Identify the \textbf{best\_score} of all candidates.
            
            \item Remove each entry from \textbf{candidates} with a difference in score and  \textbf{best\_score} greater \\ than \textbf{$\epsilon$}.
        \end{enumerate}
        
        \item Select a random entry from \textbf{candidates}.
    \end{enumerate}
 \caption{Epsilon Lexicase Selection}
 \label{alg:epsilon-lexicase}
\end{algorithm}

==> tex/scratch/alg-novelty-lexicase.tex <==
\RestyleAlgo{boxruled}
\begin{algorithm}[h!]
    \begin{enumerate}
        \setlength\itemsep{1mm}

        \item For each \textbf{case} in \textbf{text\_cases}:
        \begin{enumerate}
            \setlength\itemsep{1mm}
            \item Evaluate each member in the population on \textbf{case}.
        \end{enumerate}
        
        \item Mark the entire population as current \textbf{candidates} under consideration.
        \item Create novelty scores for each candidate in \textbf{candidates}.
        \item Update \textbf{test\_cases} to include a \textbf{case} for novelty scores.
        \item Shuffle \textbf{test\_cases} in a random order.
        \item For each \textbf{case} in \textbf{test\_cases}:
        
        \begin{enumerate}
            \setlength\itemsep{1mm}
            \item Evaluate each candidate in \textbf{candidates} on \textbf{case}.
            \item Identify the \textbf{best\_score} of all candidates.
            \item Remove each entry from \textbf{candidates} with a score less than \textbf{best\_score}.
        \end{enumerate}
            
        \item Select a random entry from \textbf{candidates}.

    \end{enumerate}
 \caption{Novelty-Lexicase Selection}
 \label{alg:novelty-lexicase}
\end{algorithm}

==> tex/scratch/broad-intro.tex <==
\section{Introduction}

% - Fitness landscapes
%   - Parent selection algorithms
%   - Parent selection algorithms in the context of fitness landscapes
%   - Analyzing selection algorithms => how do they traverse the fitness landscape?

In evolutionary computing, a fitness landscape describes the search space for a given computational problem. 
In contrast to [biological evolution], evolutionary algorithms actively direct populations through a problem's search space via repeated evaluation, selection, and variation (\textit{i.e.}, replicating promising individuals with random mutations) until a sufficiently good solution is found. 
Each of these algorithmic components---how we represent and interpret individuals, how we select which individuals to [reproduce/produce offspring/contribute genetic material to next generation], and how we [vary/mutate] offspring---are intertwined; together, these components determine how an evolutionary algorithm navigates the fitness landscape, which, in turn, determines the success of evolutionary search. 
% Many techniques exist. How do they direct populations, and how to choose which ones to use?

% JGH: If anyone has a cool paper of EAs solving hard problems feel free to cite!
Interest in evolutionary algorithms has grown over time, due to the fact that these algorithms demonstrate the ability to traverse complex fitness landscapes and produce high-quality solutions for real-world optimization problems [CITE]. 
As evolutionary algorithms continued to show promise with solving complex real-world optimization problems, the complexity of processes that occur during an evolutionary run also increased to solve even more difficult problems.
This is clearly illustrated when comparing an early evolutionary algorithm, such as the ES$(\mu, \lambda)$ Evolutionary Strategy, to a more modern algorithm, such as the MAP-Elites algorithm \cite{eiben1998evolutionary, mouret2015illuminating}.
While the procedural complexity within evolutionary algorithms continues to increase, many share a common step throughout their evolutionary search for high-quality solutions -- the selection scheme.
The selection algorithm is a crucial component to an evolutionary algorithm, as it determines what regions of the fitness landscape to explore or exploit when it selects solutions to act parents for the following generation of solutions.


% - Exploration vs. exploitation
%  - Pure exploitation (greedy algorithms)
%  - Pure exploration (enumerate all possibilities)
%   - Efficient pure exploration => novelty search
% - Striking a balance between exploitation and exploration
%  - Diversity maintenance, quality diversity algorithms

Understanding how evolutionary algorithms perform exploration and exploitation within a fitness landscape is important information to have.
As a practitioner, this information can make it possible to know what kind of evolutionary algorithm to use to meet solution requirements.
The design of an evolutionary algorithm can dictate the trade-off between exploitation and exploration, as the selection scheme and mutation operators (point mutations, crossover, \textit{etc}.) play a role in determining the strength of each one \cite{eiben1998evolutionary}.
Looking at an algorithm that is extremely exploitative, the algorithm will push the population to closest optimum, regardless of the optimum being global or local, and the population will not be able to escape it to explore promising regions of the landscape.
Now looking at the other extreme, an algorithm that is extremely exploratory will spread the population across the potentially promising regions of the fitness landscape but never reach an actually optimum.
Thus, it is clear that striking a balance between exploration and exploitation is crucial to finding high quality solutions, as it is important to exploit promising regions of the fitness landscape, while also exploring the fitness landscape to find other promising regions.
Different techniques were also created to balance exploration and exploitation, some of which include fitness sharing, novelty search, and age-layered population structure \cite{goldberg1987genetic, lehman2011novelty, hornby2006alps}.

% - Analyzing selection algorithms with benchmarking
%   - Benchmarking
%   - Often overall problem solving success of an entire system, do not isolate selection scheme
%     - Mutation rate, representation, problem, etc
%   - Very useful in how a whole system performs in practice %   - But if our interest is to characterize selection schemes, can confound results
%   - Some benchmarking uses very stripped down/limited problems, but still don't isolate individual characteristics of a selection scheme.

In practice, it is common to evaluate an problem solving potential evolutionary algorithms to get a better understanding of its strengths and weaknesses.
Often researchers evaluate an evolutionary algorithm on real-world optimization problems that inherently posses multiple interwoven challenging characteristics, such as conflicting objectives, deception, multi-modal, \textit{etc.}, that make it difficult to extract information about the kinds of problems it may be best suited for.
It is possible to visualize certain optimization problems, for example if a solution consists of a two-dimensional coordinate, but it not all problems can use such a simple underlying structure.
There is ongoing research in the field of fitness landscape analysis that focuses on the development of metrics that are able to capture characteristics that make solving an optimization problem difficult, but is limiting when the search space is extremely large \cite{malan2013survey}.
It is also common to use both fitness landscape analysis and benchmark functions to tease apart the strengths and weaknesses of evolutionary algorithms, so that practitioners can make better decisions on which one to use \cite{sun2014selection}.
One problem that occurs with using existing benchmark problems is that they too can intertwine multiple problem characteristics.
Carefully constructing and describing novel diagnostic problems can help practitioners better understand the strengths and weaknesses of an entire evolutionary algorithm, and also how the variation of specific evolutionary algorithm components (mutation rate, mutation operator, selection scheme, \textit{etc.}) impact its problem solving success.

% - Selection scheme diagnostics
%   - Can we diagnose different characteristics of selection schemes?
%   - Selection scheme diagnostics
%   - meant to complement benchmarking (different goal: isolate/understand characteristics of selection schemes)
%   - Introduce an *exploration* diagnostic designed to diagnose capacity for fitness landscape exploration
% JGH: I think this might have combined this in the previous paragraph

% - Use exploration diagnostic to investigate lexicase selection
%  - Verify intuition and previous benchmarking results showing that it better explores relative to tournament/mu lambda (very exploitative algorithms) 
%  - ?? number of test cases/problem decomposition?
%  - Investigate how different lexicase variants alter exploration
%    - Down-sampled
%    - Epsilon
%  - Investigate how addition of exploration-focused test cases can alter exploration
%    - Genotypic similarity (fitness sharing inspired)
%    - Age/generation (Age-layered population structure inspired)

In this work, we introduce a novel diagnostic that tests an evolutionary algorithms ability to explore multiple avenues within a fitness landscape, with the goal of finding the best avenue to pursue.
The total number of possible avenues is user dependent, so practitioners are also able to find where an algorithms exploratory abilities begin to fall off.
In particular, the algorithm of focus in this work is lexicase selection, along with other subsampling variations of it \cite{helmuth2014solving, hernandez2019random}.
We start by testing lexicase on this exploratory diagnostic with an increasing number of possible avenues to pursue to gain an understanding of its exploratory limitations.
We also evaluate how the different subsampling variations of lexicase impact an evolutionary algorithms ability to explore the exploratory diagnostic fitness landscape.
With all this information, we hope to highlight how the different variations of lexicase in this work impact an evolutionary algorithms problem solving ability when exploration is key to its success.  

==> tex/scratch/methods.tex <==
\section{Methods}

We conducted a series of experiments to analyze the exploratory limits of standard lexicase selection and four of its variants:
$\epsilon$-lexicase, down-sampled lexicase, cohort lexicase, and novelty lexicase. 
%difference in exploration capacity for each of the lexicase variants previously described.
In all of our experiments, we evolved populations of 500 numerical vectors on our exploration diagnostic (described in Section \ref{sec:exploration-diagnostic}) for 50,000 generations.
The initial population consisted of vectors where each value was set to 0.0, denoting the lowest point in the landscape.
% While we could have started with vectors of random sequences, we decided to have the population start from the same,lowest possible point in the landscape.

When evaluating a candidate solution, we calculate a score associated with each position in its vector according to the exploration diagnostic (Figure [XX]).
We then use this collection of scores as test case results for the purposes of lexicase selection and its variants.
If a single fitness value is required (e.g., for tournament selection), we sum the individual scores to determine the solution's aggregate fitness.

Selected candidate solutions are reproduced asexually, and we apply point-mutations to offspring at a per-position rate of 0.7\%. 
The magnitude of each mutation is drawn from a normal distribution with a mean of 0.0 and a standard deviation of 1.0 ($\mathcal{N}(0, 1)$).

% %For lexicase selection, we use each position's score as a test case. 
%When evaluating solutions, the solutions vector is scored and a fitness vector calculated.
%This fitness vector is then used by all of the previously mentioned lexicase variants, where each variant is called to select enough parents to fill the next generations population.
% Once the set of parents is constructed, we go through each position in a parent's vector and apply a point-mutation that comes from $\mathcal{N}(0, 1)$ at a rate of .7\%.
%After applying going through applying mutations to all parents, where applicable, we repeat this cycle for 50,000 generations.

% From a conceptual level, we consider the values in a candidate solution to each represent its output for a test case.
% The search space is structured such that only a consecutive group of test cases can be solved.
% The highest value overall indicates the position of the beginning of the solve group.
% Subsequent test cases are also considered solved if they are less than or equal to all of the test cases in the group that came before them.

% [Lexicase selection ...]
% [To apply lexicase, we categorize each position in a vector as pass/fail.]
% [Passing positions get their score, failing positions get a 0].

% --- BOOKMARK ---

\subsection{Verifying...}

To answer the first question, we conducted 


\subsection{Limits of lexicase exploration}

We ran experiments with an increasing number of possible avenues to pursue in order to gain insight on the limitations of lexicase's exploration capacity.
The sizes of the numerical vectors ranged from $10,20,50,100,200,500,1000$, and 50 replicates ran for each treatment.
We emphasize that by increasing the size of the vectors, the amount of exploration needed to find the best starting position is also increased. 

\subsection{Lexicase variants affect on exploration}

In order to measure the impact that each variant has on lexicase selections exploration capacity, we ran experiments comparing each variance to standard lexicase selection. 
For these experiments, all vectors were set to be a size of 100 and vary the configuration parameter of each variant.
The $\epsilon$ values for $\epsilon-$lexicase were estimated based off previous work that used $\epsilon$-lexicase to solve symbolic regression problems [cite].
The novelty-lexicase $k-$nearest neighbors were also estimated based off previous work that used standard novelty search to evolve maze solvers [cite].
Each configuration has 50 replicates and can be found in table [TODO]. \\

\begin{center}
    \begin{tabular}{ |c|c|c|c|  }
    \hline
    \multicolumn{4}{|c|}{Lexicase variant configuration list} \\
    \hline
    $\epsilon$-lexicase & Down-sampled & Cohort & Novelty\\
    \hline
    0.0  & 1\%   & 1\%   & 0\\
    0.1  & 2\%   & 2\%   & 1\\
    0.3  & 3\%   & 3\%   & 4\\
    0.6  & 12\%  & 12\%  & 8\\
    1.2  & 25\%  & 25\%  & 15\\
    2.5  & 50\%  & 50\%  & 30\\
    5.0  & 100\% & 100\% & 60\\
    10.0 &  &  & \\
    \hline
    \end{tabular}
\end{center}


%%%%%%%% WORK THIS TEXT IN?
% We obtained our epsilon values from a scaled maximum epsilon value in [cite-lex-regression].
% This gave us epsilons of different magnitudes, between the ranges of 0.0 and 10.0 to work with.
%%%%%%%%%%

==> tex/scratch/old-diagnosing-lexicase-and-its-variants.tex <==
% (1) Lexicase vs. Tournament
% \subsection{Does lexicase selection explore more than tournament selection?}

% First, we used the exploration diagnostic to test expectations that lexicase selection improves exploration relative to tournament selection.
% Unlike lexicase selection, tournament selection does not reliably maintain multiple niches within a population, and as such, we expect it to perform poorly on the exploration diagnostic relative to lexicase selection.
% In this experiment, tournament selection used tournaments of eight individuals to select parents.

% % \input{tex/figures/fig-tourny-performance-over-time}

% % Results
% In line with our expectations, we found that lexicase selection outperforms tournament selection on the exploration diagnostic (Figure \ref{fig:tournament}).
% Early on, populations evolving under tournament selection converge to a single local optimum in the exploration diagnostic (\textit{i.e.}, a single starting position), and there is no mechanism for the population to escape. 
% Lexicase selection, however, rewards specialists for different starting positions, allowing the population to continuously explore different evolutionary pathways.

% (2) The exploratory limits of lexicase selection
\subsection{Does the exploratory capacity of lexicase selection fall off as we increase cardinality?}
% The exploratory limitations of lexicase selection

Next, we evaluated standard lexicase selection on the exploration diagnostic at a range of cardinalities: 10, 20, 50, 100, 200, 500, and 1,000.
As we increase the cardinality of the exploration diagnostic, we increase the number of potential pathways that must be explored by a population to find the global optimum. 
Because increasing cardinality obscures the path to optimality, we expected lexicase selection's performance on the exploration diagnostic to degrade with increasing cardinality.



Figure \ref{fig:lexicase} shows lexicase selection's performance at each cardinality of the exploration diagnostic.
Across all cardinalities, lexicase selection improves performance from the starting performance.
% improves solution performance from the
% Lexicase selection is able to improve solution qualities across all treatments.
% Find the ordering of 10-50, don't need to do for others since they don't overlap (for bottom line)
% At XX generation, we observe no sig difference between X,Y,Z... are significantly better than..
Notably, treatments with cardinalities 10, 20, and 50 all perform near perfectly after 50,000 generations, and 100 performs relatively well, whereas the other treatments appear to need more time to converge on their maximal performance.
Thus, with the configuration of these experiments (asexual populations of 500 solutions evolved for 50,000 generations), it appears that lexicase selection is able to achieve at least a 90\% of optimal fitness on cardinalities less than or equal to 100. 
As such, all other experiments here are focused on vectors of length 100, which is sufficient for standard lexicase selection to converge at a reasonable solution, while still leaving room for improvement.

In each of the 500 selection events per generation, scores for vector positions are evaluated in a random order.
Across a population, we expect that positions that are consistently rewarded should maintain solutions that start at that position.
Since the optimal solution requires the very first position to be the highest in the population, the chance of that one being skipped (never being chosen first) in a generation will vary with cardinality.
With a population size of 500 and a vector with 50 positions, there is a 0.004\% chance (1 in 25k) of the first position being skipped, making it unlikely for it to go unselected.
Increasing the vector size to 100 positions, however, increases the chance of the first position failing to be selected to 0.657\% (1 in 152), a much more likely occurrence that may explain the reduced performance.
By vector size 200, this probability rises to 8.157\%, an even more likely occurrence.
As such, increasing the population size would allow lexicase to support higher levels of exploration.

% (3) Epsilon
\subsection{Does relaxing lexicase selection's elitism affect exploration?}
% Exploration in epsilon-lexicase selection

As discussed in Section \ref{sec:epsilon-lexicase-selection}, $\epsilon$-lexicase relaxes the elitism of lexicase selection.
To test whether this relaxation of elitism affects exploration, we compared standard lexicase selection and $\epsilon$-lexicase selection on the exploration diagnostic. 
Specifically, we evolved 50 replicates populations at each of the following $\epsilon$ values: 0.0, 0.1, 0.3, 0.6, 1.2, 2.5, 5.0, and 10.0.
Note that an $\epsilon$ value of 0.0 is identical to standard lexicase selection.

Looking at Figure \ref{fig:epsilon}, we see that $\epsilon$ values of 0.6 or less follow a similar trajectory, where they all eventually converge to the similar average performances after 30,000 generations.
There is a slight decrease in performance for the $\epsilon$ value of 1.2 and steady growth for $\epsilon$ of 2.5.
As expected, $\epsilon$ 5.0 and 10.0 performs poorly. 

\input{tex/figures/fig-epsilon-lexicase-performance-over-time}

In general, $\epsilon$ lexicase is expected to have two main advantages over standard lexicase selection \citep{la2016epsilon}:
1) it allows small amounts of noise in the evaluation data to be ignored, and
2) it prevents nearly identical scores from determining which candidate solutions win, potentially allowing greater coexistence.
While the first mechanism cannot be at play here (since all scores are deterministic), the second advantage could provide additional support solutions further along a pathway.
Indeed, this hypothesis does appear to have some support.
We see in Figure \ref{fig:epsilon-inter-fin} that $\epsilon$ values 0.1, 0.3, and 0.6 appear to produce similar performances at 50,000 generations; as for larger $\epsilon$ values, performance declines. 
We find that maximum fitness values found throughout an evolutionary run for $\epsilon$ values [XX,XX,XX] are statistically greater than standard lexicase [THIS IS BASED OFF  50 OBJECTIVES - STILL TODO FOR 100].
Solutions that begin optimizing at an earlier point in their vector now have a chance to pass the filter with other solutions that began optimizing farther down in the vector and have a slightly higher value.
Eventually when a test case that favors the solutions that began optimizing from an earlier position could win and be selected as parents.
This dynamic is neutralized if population diversity stagnates and too many similar solutions pass the same filters due to a higher $\epsilon$, leading to more randomness in selection.

% \begin{figure}[h!]
%  \centering
%  \includegraphics[width=\textwidth]{tex/images/epsilon-inter-fin-all.pdf}
%   \caption{\textbf{A comparison of average trait values for elite solutions across replicates for a range of levels of $\epsilon$ at intermediate and final generations.}
%   All candidate solutions were evolved on the exploration diagnostic, using 50 replicates for each value of $\epsilon$ (0.0, 0.1, 0.3, 0.6, 1.2, 2.5, 5.0, 10.0).
%   Plot A illustrates the performances found at 1000 generations and plot B illustrates the performances found at 50,000 generations. 
%   We left out some $\epsilon$ values as they did not have similar performances to the ones presented.}
%  \label{fig:epsilon-inter-fin}
% \end{figure}

% Future exploration: 
Other potential $\epsilon$-lexicase configurations to pursue are using the an updated $\epsilon$ value, such as the median absolute deviation (MAD) \citep{la2016epsilon}. 
This technique will update the $\epsilon$ value each generation, and is dependent on the fitness variance per individual test case.
It is possible that this could lead to better performing solutions being found, given that the $\epsilon$ value will be continuously updated. 

% (4) Down-sampled lexiase
\subsection{Does down-sampled lexicase affect exploration relative to standard lexicase selection?}
% Exploration in down-sampled lexicase selection

We compared the performance of standard lexicase to that of down-sampled lexicase at a range of sampling rates (1\%, 2\%, 3\%, 12\%, 25\%, 50\%, 100\%) on the exploration diagnostic. 
Note that the 100\% sampling rate is standard lexicase selection.

\input{tex/figures/fig-down-sampled-lexicase-performance-over-time}

Any amount of down-sampling significantly degraded lexicase selection's performance (Figure \ref{fig:down-sampled}).
% [TODO]
Down-sampled lexicase selection's drop in performance is likely attributed to mismatches between candidate solutions and the test cases that they are specialized on.
As the proportion of test cases used in each generation decreases, so too does the probability of a solution encountering the same set of test cases for multiple generations in a row.
As such, a solution has a reduced chance of encountering the test cases for which it is most optimized \citep{ferguson2020characterizing}.
These dynamics will repeatedly remove solutions while they are highly specialized due to small active regions.
Indeed, we find that performance decreases as the number of test cases in the subsamples decreases (Figure \ref{fig:down-sampled}).
In fact, any downsampling used appears to have a strong negative effect, substantially reducing performance in all cases.

% REREAD
A major reason for deciding to use down-sampled lexicase, versus lexicase selection, is because of the reduction in amount of test cases evaluations needed per candidate solution.
In Figure \ref{fig:down-sampled}, both generations and population size are consistent across treatments, and as such, each treatment represents vastly different numbers of total evaluations.
If all sampling proportions use the same amount of evaluations, it may be possible to see a boost in performance on the exploration diagnostic for the sampling proportions less than 100\%. 
[TODO OR LEAVE AS FUTURE WORK]
A modification we can incorporate within down-sampled lexicase is integrating an $\epsilon$ threshold value, similar to $\epsilon$-lexicase.

% (5) Cohort lexicase
\subsection{Does cohort lexicase affect exploration relative to standard lexicase?}
% Exploration in cohort lexicase selection

Next, we evaluated how partitioning the population and test set into cohorts affects the exploration capacity of lexicase selection.
We compared the performance of standard lexicase to that of cohort lexicase at a range of cohort sizes (given as proportions of the test case set and population): 1\%, 2\%, 3\%, 12\%, 25\%, 50\%, and 100\%. 
Note that a cohort sizes generated with a proportion of 100\%  are identical to standard lexicase selection.
For example, a 1\% cohort size results in 100 cohorts of five candidate solutions and 100 cohorts each with one test case.

\input{tex/figures/fig-cohort-lexicase-performance-over-time}

As with down-sampled lexicase, any level of cohort partitioning degrades lexicase's performance on the exploration diagnostic (Figure \ref{fig:cohort}).
However, in line with our expectations, cohort lexicase does not appear to degrade lexicase selection's performance to the same degree as down-sampling at larger cohort sizes (Figure \ref{fig:down-sampled}).

Indeed, \cite{ferguson2020characterizing} found that cohort lexicase better maintained phylogenetic diversity than down-sampled lexicase, as phylogenies coalesced less frequently under cohort lexicase selection (maintaining deeper, more divergent branches).
% Because cohort lexicase ensures the use 
% This could be due to two possibilities.


Both cohort and down-sampled lexicase offer equivalent per-generation evaluation savings, but cohort lexicase uses every test case for parent selection in every generation. 
This could play a role in problem solving success, as a test case that rewards exploration any given starting position in the exploration diagnostic is used every generation.  
At small cohort sizes, however, it is less likely that specialists are evaluated on the test cases that they are specialized on.
Looking at Figure \ref{fig:cohort}, we see that proportions greater than 12\% seem to perform well and with more time could reach the same level of performance and standard lexicase.

Similar to down-sampled lexicase, cohort lexicase reduces the amount of evaluations for a fixed number of generations and a fixed population size. 
The proportions from Figure \ref{fig:cohort} all share consistent generations, yet the number of evaluations between them is vastly different.
If all proportions are given the same amount of evaluations, it is possible that the proportions less than 100\% could achieve a boost in performance.

% (6) Novelty-lexicase
\subsection{Does novelty-lexicase affect exploration relative to standard lexicase selection?}
% Exploration in novelty-lexicase selection

We evaluated how novelty scores incorporated within lexicase selection impact the exploration capacity of lexicase selection.
We compared the performance of standard lexicase selection to that of novelty-lexicase for a range of $k$-nearest neighbors: 0, 1, 2, 4, 8, 15, 30, and 60.
Note that $k=0$ is identical to standard lexicase selection.

\input{tex/figures/fig-novelty-lexicase-performance-over-time}

% [Mention that these results do not match with our hypothesis].
In Figure \ref{fig:novelty-inter-fin}, novelty-lexicase performs similarly to standard lexicase for $k$ values less than 15 at 50,000 generations, with a slightly more substantial reduction in fitness outcomes for larger $k$ values.
In the same figure, at 1000 generations, $k=60$ has found better performing solutions than standard lexicase. 
This increase in performance at 1000 generations for $k=60$ could be due to the pressure to find novel avenues early in the run, but this affect has a negative impact towards the end of the run.
In Figure \ref{fig:novelty}, all $k$ values show an upward trends in average trait performance, with lexicase selection finding better performing solutions after about 5000 generations.
The performance slowdown of standard lexicase at early generations could be due to novelty-lexicase with $k=60$ incorporating more exploration during its evolutionary search than standard lexicase. 
At a certain generation though, a solutions that optimize from an early position in the vector is found by all treatments, but standard lexicase selection may do a better job at exploiting than $k$ values greater than 0.

% \begin{figure}[h!]
%  \centering
%  \includegraphics[width=\textwidth]{tex/images/novelty-inter-fin-all.pdf}
%   \caption{\textbf{A comparison of average trait values for elite solutions across replicates for a range of levels of novelty lexicase at intermediate and final generations.}
%   All candidate solutions were evolved on the exploration diagnostic, using 50 replicates for each value of $k$ (0, 1, 2, 4, 8, 15, 30, and 60).  Novelty scores were calculated as the average distance to the $k$ nearest neighbors.
%   Plot A illustrates the performances found at 1000 generations and plot B illustrates the performances found at 50,000 generations. }
%  \label{fig:novelty-inter-fin}
% \end{figure}

Novelty search favors solutions that are able to produce behaviors that have never been seen before.
These previous studies led us to believe that novelty-lexicase would do a better job at exploration than standard lexicase selection.
At early points we see this (Figure \ref{fig:novelty}), but novelty-selection appears to hinder lexicase selection's ability to exploit high quality solutions. 
While past work has demonstrated that novelty search is effective at producing solutions for complicated problems, the exploration diagnostic does not have any of the hidden intricacies that novelty search excels at disentangling.
Novelty search appears to thrive under conditions where there are more non-linearities between genotype and phenotype.
The underlying representation used here is simple numerical vectors, as opposed to an artificial neural network or PushGP where internal architectures can change dynamically and qualitatively different outputs are possible.
These differences in problems may shine light as to why novelty-lexicase did not outperform standard lexicase selection on the exploration diagnostic.

Indeed, it was surprising to see that at 50,000 generations that novelty-lexicase was comparable with standard lexicase in terms of performance.
Perhaps novelty-lexicase's performance results may due to using the average distance between the $k-$ nearest neighbors as a novelty metric.
This novelty metric may not provide the selection scheme with useful information regarding novelty. 
Hence, trying other novelty metrics shows that...
One modification that may increase performance would be to use a combination of novelty-lexicase and $\epsilon$-lexicase, such that similar solutions are counted as identical.
Another alteration of novelty-lexicase that can possibly help is have a proportion of the parents be selected by lexicase selection and the rest by novelty search.
This modification could allow one portion of the parents to focus on exploration (novelty search), while the other portion focuses on a mix of exploration and exploitation (lexicase selection).

==> tex/scratch/results-and-discussion.tex <==
\section{Results and discussion}

% MOVE THIS TO METHODS
% Throughout these experiments we keep track of the solution with the best fitness, which consists of the average performance across all objectives (vector positions) in the vector.
% In Figures \ref{fig:lexicase}, \ref{fig:epsilon}, \ref{fig:down-sampled}, \ref{fig:cohort}, and \ref{fig:novelty} we present these results, that are averaged out over 50 replicates per treatment.
% Each line in the figures also has a 95\% confidence interval around it.
%All parameters used by each variant can be found in Table [TODO].

% Diagnosing 
% Methods (or: What did we do?)
% Results (or: What did we see?)
% Discussion (or: What does it mean?)
% Conclusions (or: Why do we care?)
% Next Steps (or Where do we go from here?)

\subsection{[Lexicase ... exploration relative to tournament selection]}

\subsection{Lexicase exploratory limitations}

In order to gain an understanding of the exploration capacity of the standard lexicase selection procedure, we conducted experiments where we varied the number of potential pathways available by [varying vector sizes].
%We again note that as the size of the numerical vector increases, the number of possible avenues to explore and hill climb also increases.
In this experiment, we evaluate lexicase selection against the exploration diagnostic with vector sizes 10, 20, 50, 100, 200, 500, and 1,000.

\begin{figure}[h!]
 \centering
 \includegraphics[width=\textwidth]{tex/images/lexicase-varying-traits.pdf}
 \label{fig:lexicase}
 \caption{\textbf{Average position score over generations across vector sizes}.  TODO}
\end{figure}

In Figure \ref{fig:lexicase}, we illustrate lexicase selection's performance across the different vector sizes.
Lexicase selection is able to improve solution qualities across all treatments.
% Find the ordering of 10-50, don't need to do for others since they don't overlap (for bottom line)
% At XX generation, we observe no sig difference between X,Y,Z... are significantly better than..
Notably, treatments with vector sizes 10, 20, and 50 all perform near perfectly after 50,000 generations, and 100 performs relatively well, whereas the other treatments appear to need more time to converge on their maximal performance.
Thus, with the configuration of these experiments (asexual populations of 500 solutions evolved for 50,000 generations), it appears that lexicase selection is able to achieve at least a 90\% of optimal fitness on objective counts less than or equal to 100. 
As such, all other experiments here are focused on vectors of length 100, which is sufficient for standard lexicase selection to converge at a reasonable solution, while still leaving room for improvement.

In each of the 500 selection events per generation, scores for vector positions are evaluated in a random order.
Across a population, we expect that positions that are consistently rewarded should maintain solutions that start at that position.
Since the optimal solution requires the very first position to be the highest in the population, the chance of that one being skipped (never being chosen first) in a generation will vary with the vector size.
With a population size of 500 and a vector with 50 positions, there is a 0.004\% chance (1 in 25k) of the first position being skipped, making it unlikely for it to go unselected.
Increasing the vector size to 100 positions, however, increases the chance of the first position failing to be selected to 0.657\% (1 in 152), a much more likely occurrence that may explain the reduced performance.
By vector size 200, this probability rises to 8.157\%, an even more likely occurrence.
As such, increasing the population size would allow lexicase to support higher levels of exploration.

% [Discussion of what this result means. Is it expected? Unexpected? Why might we see this?]
% [Hypothesis: if we increase pop size, we could improve performance for higher vector sizes because we can more reliably maintain niches. If we decrease pop size, we could see degradation of performance.]

\subsection{$\epsilon$-Lexicase: $\epsilon$ can influence exploration potential}
% Small epsilon can produce minor improvements exploration, while large epsilon degrades exploration
% epsilon dictates exploration potential in ...

In order to evaluate how $\epsilon$-lexicase affects the exploration capacity of lexicase selection, we evaluated it on the exploration diagnostic with 100 objectives.
We conducted experiments with varying $\epsilon$ values (0.0, 0.1, 0.3, 0.6, 1.2, 2.5, 5.0, 10.0), and 50 replicates per $\epsilon$ value.
Note that an $\epsilon$ value of 0.0 is identical to standard lexicase selection.
% Redo second half of bottom sentence
Looking at Figure \ref{fig:epsilon}, we see that $\epsilon$ values of 0.6 or less follow a similar trajectory, where they all eventually converge to the similar average performances after 30,000 generations.
There is a slight decrease in performance for $\epsilon$ of 1.2 and steady growth for $\epsilon$ of 2.5.
As expected, $\epsilon$ 5.0 and 10.0 performs poorly. 

\begin{figure}[h!]
 \centering
 \includegraphics[width=\textwidth]{tex/images/epsilon-vals.pdf}
 \label{fig:epsilon}
\end{figure}

In general, $\epsilon$ lexicase is expected to have two main advantages over standard lexicase selection [CITE?]:
1) It allows small amounts of noise in the evaluation data to be ignored, and
2) it prevents nearly identical scores from determining which candidate solutions win, potentially allowing greater coexistence.
While the first mechanism cannot be at play here (since all scores are deterministic), the second advantage could provide additional support solutions further along a pathway.
Indeed, this hypothesis does appear to have some support.
We see in the Figure \ref{fig:epsilon} that low $\epsilon$ values overlap one another, with a slight edge over standard lexicase.
We find that maximum fitness values found throughout an evolutionary run for $\epsilon$ values [XX,XX,XX] are statistically greater than standard lexicase [THIS IS BASED OFF OTHER PAPER WITH 50 OBJECTIVES - STILL TODO].
%We believe that this occurred due to smaller $\epsilon$ values allowing for other solutions to pass through the filtering phase of lexicase selection.
Solutions that begin optimizing at an earlier point in their vector now have a chance to pass the filter with other solutions that began optimizing farther down in the vector and have a slightly higher value.
Eventually when a test case that favors the solutions that began optimizing from an earlier position could win and be selected as parents.
This dynamic is neutralized if population diversity stagnates and too many similar solutions pass the same filters due to a higher $\epsilon$, leading to more randomness in selection.
%: which results in a random solution to be chosen as a parent. 
%While this may be a possibility, $\epsilon$-lexicase proved to be a beneficial variant to consider when exploration is crucial to problem solving success. 

% Future exploration: 
Other potential $\epsilon$-lexicase configurations to pursue are using the an updated $\epsilon$ value, such as the median absolute deviation (MAD) [cite]. 
This technique will update the $\epsilon$ value each generation, and is dependent on the fitness variance per test case.
It is possible that this could lead to better performing solutions being found. 
Another possibility is using $\epsilon$-lexicase within other variants of lexicase (down-sampling lexicase, cohort lexicase, novelty lexicase). 
It is also possible that integrating $\epsilon$ lexicase within the other variants may help find better performing solutions.

\subsection{Down-sampling decreases exploration potential}

In order to evaluate how down-sampling of test cases affects the exploration capacity of lexicase selection, we evaluated down-sampling lexicase on the exploration diagnostic with 100 objectives.
We conducted experiments with different sampling proportions (1\%, 2\%, 3\%, 12\%, 25\%, 50\%, 100\%) relative to the number of objectives.
Note that when a sampling proportion of 100\% is identical to standard lexicase selection.
Looking at Figure \ref{fig:down-sampled}, we see that sampling proportions less than 100\% perform significantly worse than standard lexicase.
The 50\% and 25\% sampling proportions perform similarly, but the confidence intervals are wide and the average fitness fall short of 40\% of the optimal fitness. 

\begin{figure}[h!]
 \centering
 \includegraphics[width=\textwidth]{tex/images/down-sampled-proportions.pdf}
 \label{fig:down-sampled}
\end{figure}

We believe that down-sampled lexicase's drop in performance is attributed to mismatches between solutions and the test cases that they are paired with.
As the proportion of test cases used in each generation decreases, so too does the probability of a solution encountering the same set of test cases for multiple generations in a row.
As such, a solution has a reduced chance of encountering the test cases for which it is most optimized [CITE - gptp2020].
% These dynamics make it easy for solutions to lose their trajectory while hill climbing and pursing any particular avenue.
These dynamics will repeatedly remove solutions while they are highly specialized due to small active regions.
%easy for solutions to lose their trajectory before much hill climbing has occurred, reducing the number of pathways being explored.
% These dynamics will repeatedly remove solutions with small active regions and thus will only be selected by limited test cases.
% We see evidence of this effect in Figure \ref{fig:down-sampled} because as the number of test cases in the subsamples decreases, so too does the algorithm performance. 
Indeed, we find that performance decreases as the number of test cases in the subsamples decreases (Figure \ref{fig:down-sampled}).
In fact, any downsampling used appears to have a strong negative effect, substantially reducing performance in all cases.
% The best performances for subsampling (less than 100\%) is minuscule when compared to standard lexicase selection, as sampling proportions 25\% and 50\% appear to be under 40\% of the optimal fitness. 
% Therefore, we can see that down-sampling has a negative impact on lexicase selection's exploratory capacity.

A major reason for deciding to use down-sampling lexicase, versus lexicase selection, is because of the reduction in amount of test cases and evaluations needed for an individual parent selection event.
When looking at the Figure \ref{fig:down-sampled}, we must keep in mind that while the generations are similar, the number of evaluations used by each sampling proportion is vastly different.
If all sampling proportions use the same amount of evaluations, it may be possible to see a boost in performance for the sampling proportions less than 100\%. 
[WE FIND THIS LATER OR LEAVE AS FUTURE WORK]
Another alteration we can use within down-sampling lexicase is incorporating an $\epsilon$ threshold value, similar to $\epsilon$-lexicase.

\subsection{Cohorts decreases exploration potential, but not as much as down-sampling}

In order to evaluate how partitioning the population and set of test cases affects the exploration capacity of lexicase selection, we evaluate cohort lexicase selection on the exploration diagnostic with 100 objectives. 
We conducted experiments with different cohort sizes that are dependent on a proportion (1\%, 2\%, 3\%, 12\%, 25\%, 50\%, 100\%) on the size of the population and test case set.
Note that cohort sizes with a proportion of 100\%  is identical to standard lexicase selection.
For cohort sizes with other proportions, looking at 1\% for example, population cohorts are of size 5 and test case cohorts are of size 1, and there are 100 cohorts for each.
Looking at Figure \ref{fig:cohort}, we see that proportions greater than 12\% seem to perform well and with more time could reach the same level of performance and standard lexicase.
the other proportion appear to be gradually increasing as well. 

\begin{figure}[h!]
 \centering
 \includegraphics[width=\textwidth]{tex/images/cohort-proportions.pdf}
 \label{fig:cohort}
\end{figure}

We believe that the higher proportion values for cohort lexicase are a major contributor to the high performance for those treatments. 
This could be due to two possibilities. 
The first possibility is due to the nature of cohort lexicase, where all the test cases are being used; unlike down-sampled lexicase where some are left out each generation. 
This could play a role in problem solving success, as solutions have the possibility of being paired up with favorable test cases.
The second possibility is due to high proportion values for cohort lexicase. 
This could play a role as well, due to solutions have a better chance of being paired up with favorable test cases as the proportion increase.

As previously mentioned, cohort lexicase reduces the amount of evaluations for a given number of generations, compared to standard lexicase selection. 
Another angle to look at this problem, is instead of giving each the same amount of generations, we give them the same amount of evaluations.
This will give us insight on the evolutionary search and exploratory abilities of down-sampled lexicase. 

\subsection{Novelty}

\begin{figure}[h!]
 \centering
 \includegraphics[width=\textwidth]{tex/images/novelty-vals.pdf}
 \label{fig:novelty}
\end{figure}


%%%%%%% SOME TEXT MOVED FROM ELSEWHERE
% - As the test cases for the early positions of the vector come up, the solutions that began optimizing in this region will be selected over the solutions who's starting position is later in the vector.

==> tex/scratch/scratch.tex <==

% -- genetic programming --
% In genetic programming (GP), we apply the natural principles of evolution to automatically synthesize computer programs to solve computational problems. 
% Genetic programming (GP) applies evolutionary search to automatically synthesize computer programs to solve computational problems.
% In the context of GP, fitness landscapes encompass all possible programs, and their ``height'' in the landscape corresponds to the quality of their performance on a given problem.
% Understanding how a particular GP system directs populations through fitness landscapes informs our [understanding] of the system's capabilities and how we might best improve them.
% At a minimum, any given GP system uses a particular program representation, one or more representation-compatible mutation operators, and a parent selection algorithm.  
% Combined, these components interact to influence how a GP system steers populations through the fitness landscape. 
% How do we disentangle the evolutionary effects of each component within a GP system? 


% For example, for a given GP system, is our choice of representation or our choice of selection scheme underlying problem-solving success? 

% Fitness landscapes in GP are complex and it can be especially challenging to study how a GP system directs populations through landscape. 
% more challenging is to disentangle each algorithmic component's contribution to how a population traverses a fitness landscape. 
% interactions between components => e.g., mutation and representation often tied tightly together
% by aggregating many benchmarking results we can begin to get a picture
% Here, we focus on parent selection, specifically. 


% that within a designated threshold 

% With standard lexicase, only solutions that share them similar top performance on a testcase do not get filtered out and epsilon lexicase relaxes this condition.
% The epsilon value provides some threshold between the optimal performance on the testcase at hand, ultimately allowing solutions that perform relatively similar to the optimal solutions. 
% There are also variations of ways to implement the epsilon value, where it can be can be a proportion of the optimal performance on a testcase or a hard-coded value.
% Epsilon lexicase demonstrated the ability to perform well on symbolic regression, and more details on this method can be found at \citep{la2016epsilon}.

% We hypothesize that as the epsilon value increases pass a certain point, there will be a decrease in performance as all test case performances are viewed as similar and pass through the filtering phase.


% We expect small $\epsilon$ to 

% \citep{

% hypothesize that small epsilon values will allow for better better solutions to be found, as solutions with similar performances on a given test case can pass through the filtering phase.
% [Maybe this goes here: how do we expect epsilon lexicase to affect exploration?]
% @AML: how does epsilon lexicase affect diversity maintenance? how do we expect epsilon to affect exploration? None? Improve? Hurt?
% Too big of an epsilon... High epsilon blurs all pathways together. 
% Smaller amounts of noise could also allow for new pathways to develop over time.
